FedGrAINS: Personalized SubGraph Federated Learning with Adaptive Neighbor Sampling

Graphs are crucial for modeling relational and biological data. As datasets grow larger in real-world scenarios, the risk of exposing sensitive information increases, making privacy-preserving training methods like federated learning (FL) essential to ensure data security and compliance with privacy regulations. Recently proposed personalized subgraph FL methods have become the de-facto standard for training personalized Graph Neural Networks (GNNs) in a federated manner while dealing with the missing links across clients' subgraphs due to privacy restrictions. However, personalized subgraph FL faces significant challenges due to the heterogeneity in client subgraphs, such as degree distributions among the nodes, which complicate federated training of graph models. To address these challenges, we propose \textit{FedGrAINS}, a novel data-adaptive and sampling-based regularization method for subgraph FL. FedGrAINS leverages generative flow networks (GFlowNets) to evaluate node importance concerning clients' tasks, dynamically adjusting the message-passing step in clients' GNNs. This adaptation reflects task-optimized sampling aligned with a trajectory balance objective. Experimental results demonstrate that the inclusion of \textit{FedGrAINS} as a regularizer consistently improves the FL performance compared to baselines that do not leverage such regularization.

==> fedgrains_arxiv <==
\begin{thebibliography}{10}

\bibitem{ahmed2023simple}
{\sc K.~Ahmed, Z.~Zeng, M.~Niepert, and G.~V. den Broeck}, {\em {SIMPLE}: A gradient estimator for k-subset sampling}, in The Eleventh International Conference on Learning Representations, 2023.

\bibitem{alam2023fedaiot}
{\sc S.~Alam, T.~Zhang, T.~Feng, H.~Shen, Z.~Cao, D.~Zhao, J.~Ko, K.~Somasundaram, S.~S. Narayanan, S.~Avestimehr, et~al.}, {\em Fedaiot: A federated learning benchmark for artificial intelligence of things}, arXiv preprint arXiv:2310.00109,  (2023).

\bibitem{arivazhagan2019federated}
{\sc M.~G. Arivazhagan, V.~Aggarwal, A.~K. Singh, and S.~Choudhary}, {\em Federated learning with personalization layers}, 2019.

\bibitem{FEDPUB}
{\sc J.~Baek, W.~Jeong, J.~Jin, J.~Yoon, and S.~J. Hwang}, {\em Personalized subgraph federated learning}, in Proceedings of the 40th International Conference on Machine Learning, 2023, pp.~1396--1415.

\bibitem{gmt}
{\sc J.~Baek, M.~Kang, and S.~J. Hwang}, {\em Accurate learning of graph representations with graph multiset pooling}, in 9th International Conference on Learning Representations, {ICLR} 2021, Virtual Event, Austria, May 3-7, 2021, 2021.

\bibitem{bengio2021flow}
{\sc E.~Bengio, M.~Jain, M.~Korablyov, D.~Precup, and Y.~Bengio}, {\em Flow network based generative models for non-iterative diverse candidate generation}, Advances in Neural Information Processing Systems, 34 (2021), pp.~27381--27394.

\bibitem{bengio2021gflow-fundation}
{\sc Y.~Bengio, S.~Lahlou, T.~Deleu, E.~J. Hu, M.~Tiwari, and E.~Bengio}, {\em Gflownet foundations}, arXiv preprint arXiv:2111.09266,  (2021).

\bibitem{blondel2008fast}
{\sc V.~D. Blondel, J.-L. Guillaume, R.~Lambiotte, and E.~Lefebvre}, {\em Fast unfolding of communities in large networks}, Journal of statistical mechanics: theory and experiment, 2008 (2008), p.~P10008.

\bibitem{fedgraph}
{\sc F.~Chen, P.~Li, T.~Miyazaki, and C.~Wu}, {\em Fedgraph: Federated graph learning with intelligent sampling}, IEEE Transactions on Parallel \& Distributed Systems, 33 (2022), pp.~1775--1786.

\bibitem{fallah2020personalized}
{\sc A.~Fallah, A.~Mokhtari, and A.~Ozdaglar}, {\em Personalized federated learning with theoretical guarantees: A model-agnostic meta-learning approach}, Advances in neural information processing systems, 33 (2020), pp.~3557--3568.

\bibitem{fang2023dropmessage}
{\sc T.~Fang, Z.~Xiao, C.~Wang, J.~Xu, X.~Yang, and Y.~Yang}, {\em Dropmessage: Unifying random dropping for graph neural networks}, in Proceedings of the AAAI Conference on Artificial Intelligence, vol.~37, 2023.

\bibitem{MPNN}
{\sc J.~Gilmer, S.~S. Schoenholz, P.~F. Riley, O.~Vinyals, and G.~E. Dahl}, {\em Neural message passing for quantum chemistry}, in Proceedings of the 34th International Conference on Machine Learning, {ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017, vol.~70 of Proceedings of Machine Learning Research, {PMLR}, 2017, pp.~1263--1272.

\bibitem{Community1}
{\sc M.~Girvan and M.~E.~J. Newman}, {\em Community structure in social and biological networks}, Proceedings of the National Academy of Sciences, 99 (2002), pp.~7821--7826.

\bibitem{GraphSAGE}
{\sc W.~Hamilton, Z.~Ying, and J.~Leskovec}, {\em Inductive representation learning on large graphs}, in Advances in Neural Information Processing Systems, I.~Guyon, U.~V. Luxburg, S.~Bengio, H.~Wallach, R.~Fergus, S.~Vishwanathan, and R.~Garnett, eds., vol.~30, Curran Associates, Inc., 2017.

\bibitem{GNN}
{\sc W.~L. Hamilton}, {\em Graph representation learning}, Synthesis Lectures on Artificial Intelligence and Machine Learning, 14 (2020), pp.~1--159.

\bibitem{spectralgraph}
{\sc D.~K. Hammond, P.~Vandergheynst, and R.~Gribonval}, {\em Wavelets on graphs via spectral graph theory}, Applied and Computational Harmonic Analysis, 30 (2011), pp.~129--150.

\bibitem{hasanzadeh2020bayesian}
{\sc A.~Hasanzadeh, E.~Hajiramezanali, S.~Boluki, M.~Zhou, N.~Duffield, K.~Narayanan, and X.~Qian}, {\em Bayesian graph neural networks with adaptive connection sampling}, in International conference on machine learning, PMLR, 2020, pp.~4094--4104.

\bibitem{fedgkt}
{\sc C.~He, M.~Annavaram, and S.~Avestimehr}, {\em Group knowledge transfer: Federated learning of large cnns at the edge}, Advances in Neural Information Processing Systems, 33 (2020), pp.~14068--14080.

\bibitem{he2021fedgraphnn}
{\sc C.~He, K.~Balasubramanian, E.~Ceyani, C.~Yang, H.~Xie, L.~Sun, L.~He, L.~Yang, P.~S. Yu, Y.~Rong, et~al.}, {\em Fedgraphnn: A federated learning system and benchmark for graph neural networks}, arXiv preprint arXiv:2104.07145,  (2021).

\bibitem{SpreadGNN}
{\sc C.~He, E.~Ceyani, K.~Balasubramanian, M.~Annavaram, and S.~Avestimehr}, {\em Spreadgnn: Serverless multi-task federated learning for graph neural networks}, AAAI,  (2022).

\bibitem{FJORD}
{\sc S.~Horvath, S.~Laskaridis, M.~Almeida, I.~Leontiadis, S.~Venieris, and N.~Lane}, {\em Fjord: Fair and accurate federated learning under heterogeneous targets with ordered dropout}, Advances in Neural Information Processing Systems, 34 (2021), pp.~12876--12889.

\bibitem{ogb}
{\sc W.~Hu, M.~Fey, M.~Zitnik, Y.~Dong, H.~Ren, B.~Liu, M.~Catasta, and J.~Leskovec}, {\em Open graph benchmark: Datasets for machine learning on graphs}, Advances in neural information processing systems, 33 (2020), pp.~22118--22133.

\bibitem{huijben2022review-gumbel}
{\sc I.~A. Huijben, W.~Kool, M.~B. Paulus, and R.~J. Van~Sloun}, {\em A review of the gumbel-max trick and its extensions for discrete stochasticity in machine learning}, IEEE Transactions on Pattern Analysis and Machine Intelligence, 45 (2022), pp.~1353--1371.

\bibitem{edge}
{\sc J.~Jo, J.~Baek, S.~Lee, D.~Kim, M.~Kang, and S.~J. Hwang}, {\em Edge representation learning with hypergraphs}, in Advances in Neural Information Processing Systems, M.~Ranzato, A.~Beygelzimer, Y.~Dauphin, P.~Liang, and J.~W. Vaughan, eds., vol.~34, Curran Associates, Inc., 2021, pp.~7534--7546.

\bibitem{Karypis95metis}
{\sc G.~Karypis}, {\em Metis: Unstructured graph partitioning and sparse matrix ordering system}, Technical report,  (1997).

\bibitem{karypis1998fast}
{\sc G.~Karypis and V.~Kumar}, {\em A fast and high quality multilevel scheme for partitioning irregular graphs}, SIAM Journal on scientific Computing, 20 (1998), pp.~359--392.

\bibitem{Adam}
{\sc D.~P. Kingma and J.~Ba}, {\em Adam: {A} method for stochastic optimization}, in 3rd International Conference on Learning Representations, {ICLR} 2015, San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings, 2015.

\bibitem{GCN}
{\sc T.~N. Kipf and M.~Welling}, {\em Semi-supervised classification with graph convolutional networks}, in 5th International Conference on Learning Representations, {ICLR} 2017, Toulon, France, April 24-26, 2017, Conference Track Proceedings, 2017.

\bibitem{kool2019stochastic}
{\sc W.~Kool, H.~Van~Hoof, and M.~Welling}, {\em Stochastic beams and where to find them: The gumbel-top-k trick for sampling sequences without replacement}, in International Conference on Machine Learning, PMLR, 2019, pp.~3499--3508.

\bibitem{li2023less}
{\sc J.~Li, S.~Tian, R.~Wu, L.~Zhu, W.~Zhao, C.~Meng, L.~Chen, Z.~Zheng, and H.~Yin}, {\em Less can be more: Unsupervised graph pruning for large-scale dynamic graphs}, arXiv preprint arXiv:2305.10673,  (2023).

\bibitem{li2018deeper}
{\sc Q.~Li, Z.~Han, and X.-M. Wu}, {\em Deeper insights into graph convolutional networks for semi-supervised learning}, in Proceedings of the AAAI conference on artificial intelligence, vol.~32, 2018.

\bibitem{FLsurvey}
{\sc Q.~Li, Z.~Wen, Z.~Wu, S.~Hu, N.~Wang, Y.~Li, X.~Liu, and B.~He}, {\em A survey on federated learning systems: vision, hype and reality for data privacy and protection}, IEEE Transactions on Knowledge and Data Engineering,  (2021).

\bibitem{li2020federated}
{\sc T.~Li, A.~K. Sahu, M.~Zaheer, M.~Sanjabi, A.~Talwalkar, and V.~Smith}, {\em Federated optimization in heterogeneous networks}, in Proceedings of Machine Learning and Systems 2020, MLSys 2020, Austin, TX, USA, March 2-4, 2020, mlsys.org, 2020.

\bibitem{malkin2022trajectorybalance}
{\sc N.~Malkin, M.~Jain, E.~Bengio, C.~Sun, and Y.~Bengio}, {\em Trajectory balance: Improved credit assignment in gflownets}, Advances in Neural Information Processing Systems, 35 (2022), pp.~5955--5967.

\bibitem{malkin2022gflownets-off}
{\sc N.~Malkin, S.~Lahlou, T.~Deleu, X.~Ji, E.~Hu, K.~Everett, D.~Zhang, and Y.~Bengio}, {\em Gflownets and variational inference}, arXiv preprint arXiv:2210.00580,  (2022).

\bibitem{amazon}
{\sc J.~McAuley, C.~Targett, Q.~Shi, and A.~Van Den~Hengel}, {\em Image-based recommendations on styles and substitutes}, in Proceedings of the 38th international ACM SIGIR conference on research and development in information retrieval, 2015, pp.~43--52.

\bibitem{McMahan2017CommunicationEfficientLO}
{\sc H.~B. McMahan, E.~Moore, D.~Ramage, S.~Hampson, and B.~A. y~Arcas}, {\em Communication-efficient learning of deep networks from decentralized data}, in AISTATS, 2017.

\bibitem{gaflow}
{\sc L.~Pan, D.~Zhang, A.~Courville, L.~Huang, and Y.~Bengio}, {\em Generative augmented flow networks}, in The Eleventh International Conference on Learning Representations, 2023.

\bibitem{Community}
{\sc F.~Radicchi, C.~Castellano, F.~Cecconi, V.~Loreto, and D.~Parisi}, {\em Defining and identifying communities in networks}, Proceedings of the national academy of sciences, 101 (2004), pp.~2658--2663.

\bibitem{Rong2020DropEdge}
{\sc Y.~Rong, W.~Huang, T.~Xu, and J.~Huang}, {\em Dropedge: Towards deep graph convolutional networks on node classification}, in International Conference on Learning Representations, 2020.

\bibitem{sattler2020clustered}
{\sc F.~Sattler, K.-R. M{\"u}ller, and W.~Samek}, {\em Clustered federated learning: Model-agnostic distributed multitask optimization under privacy constraints}, IEEE transactions on neural networks and learning systems, 32 (2020), pp.~3710--3722.

\bibitem{planetoid}
{\sc P.~Sen, G.~Namata, M.~Bilgic, L.~Getoor, B.~Galligher, and T.~Eliassi-Rad}, {\em Collective classification in network data}, AI magazine, 29 (2008), pp.~93--93.

\bibitem{amnazonsubset}
{\sc O.~Shchur, M.~Mumme, A.~Bojchevski, and S.~G{\"u}nnemann}, {\em Pitfalls of graph neural network evaluation}, arXiv preprint arXiv:1811.05868,  (2018).

\bibitem{dropout}
{\sc N.~Srivastava, G.~Hinton, A.~Krizhevsky, I.~Sutskever, and R.~Salakhutdinov}, {\em Dropout: A simple way to prevent neural networks from overfitting}, Journal of Machine Learning Research, 15 (2014), pp.~1929--1958.

\bibitem{graphfl}
{\sc Y.~Tan, Y.~Liu, G.~Long, J.~Jiang, Q.~Lu, and C.~Zhang}, {\em Federated learning on non-iid graphs via structural knowledge sharing}, arXiv preprint arXiv:2211.13009,  (2022).

\bibitem{graphflsystem}
{\sc Z.~Wang, W.~Kuang, Y.~Xie, L.~Yao, Y.~Li, B.~Ding, and J.~Zhou}, {\em Federatedscope-gnn: Towards a unified, comprehensive and efficient package for federated graph learning}, in {KDD} '22: The 28th {ACM} {SIGKDD} Conference on Knowledge Discovery and Data Mining, Washington, DC, USA, August 14 - 18, 2022, A.~Zhang and H.~Rangwala, eds., {ACM}, 2022, pp.~4110--4120.

\bibitem{FedGNN}
{\sc C.~Wu, F.~Wu, Y.~Cao, Y.~Huang, and X.~Xie}, {\em Fedgnn: Federated graph neural network for privacy-preserving recommendation}, KDD,  (2021).

\bibitem{GNN/2}
{\sc Z.~Wu, S.~Pan, F.~Chen, G.~Long, C.~Zhang, and P.~S. Yu}, {\em A comprehensive survey on graph neural networks}, {IEEE} Trans. Neural Networks Learn. Syst., 32 (2021), pp.~4--24.

\bibitem{GCFL}
{\sc H.~Xie, J.~Ma, L.~Xiong, and C.~Yang}, {\em Federated graph classification over non-iid graphs}, in Advances in Neural Information Processing Systems, vol.~34, Curran Associates, Inc., 2021, pp.~18839--18852.

\bibitem{xie2019reparameterizable}
{\sc S.~M. Xie and S.~Ermon}, {\em Reparameterizable subset sampling via continuous relaxations}, arXiv preprint arXiv:1901.10517,  (2019).

\bibitem{FedGCN}
{\sc Y.~Yao and C.~Joe{-}Wong}, {\em Fedgcn: Convergence and communication tradeoffs in federated training of graph convolutional networks}, arXiv preprint arXiv:2201.12433,  (2022).

\bibitem{FedSage}
{\sc K.~Zhang, C.~Yang, X.~Li, L.~Sun, and S.~M. Yiu}, {\em Subgraph federated learning with missing neighbor generation}, in Advances in Neural Information Processing Systems, vol.~34, Curran Associates, Inc., 2021, pp.~6671--6682.

\bibitem{GNN/1}
{\sc J.~Zhou, G.~Cui, S.~Hu, Z.~Zhang, C.~Yang, Z.~Liu, L.~Wang, C.~Li, and M.~Sun}, {\em Graph neural networks: {A} review of methods and applications}, {AI} Open, 1 (2020), pp.~57--81.

\end{thebibliography}


==> sections/table-disjoint-drop.tex <==
\begin{table*}[t]
\caption{\small \textbf{Results on the disjoint node scenario.} The reported results are mean and standard deviation over three different runs. The statistically significant performances ($p > 0.05$) are emphasized in bold.}
\label{tab:main:nonoverlap}
\small
\centering
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{\bf Cora} & \multicolumn{3}{c}{\bf CiteSeer} & \multicolumn{3}{c}{\bf PubMed}  \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-11}
\textbf{Methods} & \textbf{5 Clients} & \textbf{10 Clients} & \textbf{20 Clients} & \textbf{5 Clients} & \textbf{10 Clients} & \textbf{20 Clients} & \textbf{5 Clients} & \textbf{10 Clients} & \textbf{20 Clients}  \\
\midrule


FedAvg & 79.63 $\pm$ 4.37 &
72.06 $\pm$ 2.18 &
69.50 $\pm$ 3.58 &
70.24 $\pm$ 0.47 &
68.32 $\pm$ 2.59 &
65.12 $\pm$ 2.15 &
84.87 $\pm$ 0.41 &
78.92 $\pm$ 0.39 &
78.21 $\pm$ 0.25 \\

FedGDrop (with local GFN) &  82.92 $\pm$ 1.11  & 80.16 $\pm$ 1.62  & 81.17 $\pm$ 1.22 & 73.09 $\pm$ 1.55  & 74.63 $\pm$ 1.35 & 70.19 $\pm$ 2.55 &85.83  $\pm$ 0.35  & 85.72 $\pm$  0.46& 84.39 $\pm$ 0.46  \\


\midrule

& \multicolumn{3}{c}{\bf Amazon-Computer} & \multicolumn{3}{c}{\bf Amazon-Photo} & \multicolumn{3}{c}{\bf ogbn-arxiv}  \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-11}
\textbf{Methods} & \textbf{5 Clients} & \textbf{10 Clients} & \textbf{20 Clients} & \textbf{5 Clients} & \textbf{10 Clients} & \textbf{20 Clients} & \textbf{5 Clients} & \textbf{10 Clients} & \textbf{20 Clients} \\
\midrule

Local  & 89.18 $\pm$ 0.15 &  88.25 $\pm$ 0.21 & 84.34 $\pm$ 0.28 &
91.85 $\pm$ 0.12 & 89.56 $\pm$ 0.09 & 85.83 $\pm$ 0.17 & 66.87 $\pm$ 0.09 & 66.03 $\pm$ 0.14
& 65.43 $\pm$ 0.21 \\

\midrule

FedAvg  & 88.03 $\pm$ 1.68 &
81.82 $\pm$ 1.71 &
78.19 $\pm$ 0.86 &
89.26 $\pm$ 1.80 &
85.31 $\pm$ 1.67 &
82.59 $\pm$ 1.18 &
66.24 $\pm$ 0.45 &
64.09 $\pm$ 0.83  &
62.47 $\pm$ 1.19 \\
FedGDrop (with local GFN)   &  87.59 $\pm$ 0.66  & 89.21 $\pm$ 0.42  & 88.18 $\pm$ 0.11 & 92.95 $\pm$ 0.29 & 91.48 $\pm$ 0.60 & 90.60 $\pm$ 0.79 & -  & - & -   \\ \midrule



\bottomrule
\end{tabular}
}
\end{table*}


% FedGDrop (with Fed GFN)   &  87.69 $\pm$ 0.69  & 89.07 $\pm$ 0.50  & 88.38 $\pm$ 0.59 & 92.53 $\pm$ 0.29  & 91.40 $\pm$ 0.48 & 90.83 $\pm$ 0.68 &-  & - & -  \\

==> sections/table-overlap-drop.tex <==

\begin{table*}[t]
\caption{\small \textbf{Results on the overlapping node scenario.} The reported results are mean and standard deviation over three different runs. The statistically significant performances ($p > 0.05$) are emphasized in bold.}
\label{tab:main:overlap}
\small
\centering
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{\bf Cora} & \multicolumn{3}{c}{\bf CiteSeer} & \multicolumn{3}{c}{\bf Pubmed}  \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-11}
\textbf{Methods} & \textbf{10 Clients} & \textbf{30 Clients} & \textbf{50 Clients} & \textbf{10 Clients} & \textbf{30 Clients} & \textbf{50 Clients} & \textbf{10 Clients} & \textbf{30 Clients} & \textbf{50 Clients} \\
\midrule


FedAvg  & 78.55 $\pm$ 0.49 & 69.56 $\pm$ 0.79 & 65.19 $\pm$ 3.88 & 68.73 $\pm$ 0.46 & 65.02 $\pm$ 0.59
& 63.85 $\pm$ 1.31 & 84.66 $\pm$ 0.11 & 80.62 $\pm$ 0.46 & 80.18 $\pm$ 0.50 \\
FedGDrop (with Fed GFN)   & 79.77 $\pm$ 1.05 & 76.88 $\pm$ 1.73 & 79.20 $\pm$ 2.54 & 70.53 $\pm$ 1.06 & 69.81 $\pm$ 1.78 & 70.02 $\pm$ 2.95 & 84.57 $\pm$ 0.43 & 84.24 $\pm$ 0.59 & 83.91 $\pm$ 0.61 \\
FedGDrop (with local GFN) & 79.52 $\pm$ 1.25  & 76.99 $\pm$ 1.69  & 79.45 $\pm$ 2.28 & 70.50 $\pm$ 0.93 & 69.80 $\pm$ 1.78 & 70.33 $\pm$ 2.47 & 84.59 $\pm$ 0.35& 84.32 $\pm$ 0.51 & 83.85 $\pm$ 0.69  \\
\midrule
FedGDrop (with locGFN + PerAgg)   &  81.48 $\pm$ 0.23  & 77.85 $\pm$ 0.41  & 75.71 $\pm$ 0.33 & 71.95 $\pm$ 0.37 & 68.45 $\pm$ 0.40 & 67.25 $\pm$ 0.59 & -  & - \\ \midrule
FedPer  & 78.84 $\pm$ 0.32 &
73.46 $\pm$ 0.43 & 
72.54 $\pm$ 0.52 & 
70.42 $\pm$ 0.26 & 
65.09 $\pm$ 0.48 &
64.04 $\pm$ 0.46 & 
85.76 $\pm$ 0.14 & 
83.45 $\pm$ 0.15 &
81.90 $\pm$ 0.23 \\ \midrule
GCFL+    & 78.60  $\pm$ 0.25 & 
73.41  $\pm$ 0.36 & 
73.13  $\pm$ 0.87 &
69.80  $\pm$ 0.34 &
65.17  $\pm$ 0.32 &
64.71  $\pm$ 0.67 & 
85.08  $\pm$ 0.21 & 
83.77  $\pm$ 0.17 & 
80.95  $\pm$ 0.22  \\

GCFL+  w FedGDrop   & 79.63 $\pm$ 1.01 & 77.01 $\pm$ 1.81 & 79.81 $\pm$ 2.82 & 70.15 $\pm$ 1.80 & 69.29 $\pm$ 1.77 & 70.45 $\pm$ 2.66 & 84.51 $\pm$ 0.34  & 84.25 $\pm$ 0.62 & 83.81 $\pm$ 0.62 \\ \midrule
FedSage+ & 79.01 $\pm$ 0.30  & 
72.20 $\pm$ 0.76 & 
66.52 $\pm$ 1.37 & 
70.09 $\pm$ 0.26 &
66.71 $\pm$ 0.18 & 
64.89 $\pm$ 0.25 &
86.07 $\pm$ 0.06 & 
83.26 $\pm$ 0.08 &
80.48 $\pm$ 0.20  \\ 
\midrule
FED-PUB   & 79.65 $\pm$  0.17 & 
75.42 $\pm$  0.48 &
73.13 $\pm$  0.29 &
70.43 $\pm$  0.27 &
67.41 $\pm$  0.36 & 
65.13 $\pm$  0.40 & 
85.60 $\pm$  0.10& 
85.19 $\pm$  0.15& 
84.26 $\pm$  0.19 \\



\midrule

& \multicolumn{3}{c}{\bf Amazon-Computer} & \multicolumn{3}{c}{\bf Amazon-Photo} & \multicolumn{3}{c}{\bf ogbn-arxiv}  \\
\cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-11}
\textbf{Methods} & \textbf{10 Clients} & \textbf{30 Clients} & \textbf{50 Clients} & \textbf{10 Clients} & \textbf{30 Clients} & \textbf{50 Clients} & \textbf{10 Clients} & \textbf{30 Clients} & \textbf{50 Clients} \\
\midrule

Local   & 88.50 $\pm$ 0.20 & 86.66 $\pm$ 0.00 & 87.04 $\pm$ 0.02 & 92.17 $\pm$ 0.12 & 90.16 $\pm$ 0.12 & 90.42 $\pm$ 0.15 & 62.52 $\pm$ 0.07 & 61.32 $\pm$ 0.04 & 60.04 $\pm$ 0.04 \\

\midrule

FedAvg  & 88.99 $\pm$ 0.19 & 83.37 $\pm$ 0.47 & 76.34 $\pm$ 0.12 & 92.91 $\pm$ 0.07 & 89.30 $\pm$ 0.22 & 74.19 $\pm$ 0.57 & 63.56 $\pm$ 0.02 & 59.72 $\pm$ 0.06 & 60.94 $\pm$ 0.24 \\

FedGDrop (with Fed GFN)   &  87.51 $\pm$ 0.38  & 86.18 $\pm$ 0.66  & 87.75 $\pm$ 0.82 & 92.19 $\pm$ 4.35 & 91.14 $\pm$ 0.55 & 89.98 $\pm$ 1.21 &-  & - & -  & - \\
FedGDrop (with local GFN)   &  87.70 $\pm$ 0.41  & 86.26 $\pm$ 0.62 & 87.85 $\pm$ 1.19 & 92.66 $\pm$ 0.38 & 91.05 $\pm$ 0.52 & 89.92 $\pm$ 0.96 &-  & - & -   \\ \midrule

\bottomrule

\end{tabular}
}
\end{table*}
